Discovering Latent Concepts Learned in BERT

A large number of studies that analyze deep neural network models and their ability to encode various linguistic and non-linguistic concepts provide an interpretation of the inner mechanics of these models. The scope of the analyses is limited to pre-defined concepts that reinforce the traditional linguistic knowledge and do not reflect on how novel concepts are learned by the model. We address this limitation by discovering and analyzing latent concepts learned in neural network models in an unsupervised fashion and provide interpretations from the model's perspective. In this work, we study: i) what latent concepts exist in the pre-trained BERT model, ii) how the discovered latent concepts align or diverge from classical linguistic hierarchy and iii) how the latent concepts evolve across layers. Our findings show: i) a model learns novel concepts (e.g. animal categories and demographic groups), which do not strictly adhere to any pre-defined categorization (e.g. POS, semantic tags), ii) several latent concepts are based on multiple properties which may include semantics, syntax, and morphology, iii) the lower layers in the model dominate in learning shallow lexical concepts while the higher layers learn semantic relations and iv) the discovered latent concepts highlight potential biases learned in the model. We also release a novel BERT ConceptNet dataset (BCN) consisting of 174 concept labels and 1M annotated instances.

==> conceptpool_story.tex <==
\section{What is a concept?}
\label{sec:concept}
The goal of interpretation is to analyze representations of a model with respect to a concept. 
The previous work on interpretation mainly used human-defined language concepts such as parts of speech tags and semantic tags, thus the definition of concept surrounds around what is linguistically categorized.  
%However, due to the easy access to human-defined concepts such as parts of speech tags, semantic tags, the previous work on interpretation mainly analyze models with respect to them. 
For latent concepts learned in the model, it is difficult to come up with a precise definition of concept~\citep{concept_possession}. \citet{NEURIPS2019_kim_concept} made an attempt in defining  concept for vision models and introduced a set of properties that a concept should possess. Here, we follow their footsteps and adapt their definition to NLP.

\begin{itemize}
    \item \textbf{Meaningfulness} A group of words that are related semantically, syntactically or morphologically. For example, names of ice hockey teams form a semantic cluster, words that occur in the first position of a sentence are syntactically related.
    \item \textbf{Coherence} A group of words should have a coherent relationship among each other and they are different from other groups of words. For example, names of ice hockey teams split into two group have coherence within group but two groups might not be different from each other.
\end{itemize}

A group of words that do not possess one or more above defined properties does not imply that the grouping is wrong. Instead we mark it an uninterpretable cluster. There may exist a relation that annotators are unable to comprehend. Note that the properties specified above provides an imprecise definition of a concept and there can be certain cases and properties that may not be covered by the current definition.

\section{Related Work}


\section{Methodology}
\section{First story }
Consider a neural network model $\modelM$ with $L$ layers ${l_1, l_2 , ..., l_L}$. Our goal is to analyze latent concepts learned in various layers of $\modelM$. 
Let $\dataD$ be a dataset composed of $S$ sentences where each sentence consists of $M$ words $w_1, w_2, ..., w_M$. We extract layer-wise contextualized representation of each word $w_i$ in sentences $S$. For each layer, we cluster words into $K$ groups using their contextualized representations. We use agglomerative hierarchical clustering with \textcolor{red}{average linkage}. We call these groups of words as \emph{concept-candidates}. Each concept candidate present a latent concept that the model has learned about the language.

\subsection{Concept Selection}
The next step is to select concepts from the concept-candidates that fits in our definition of concepts. Ideally a human annotator goes over the candidates and filter out uniterpretable concepts. However, doing this for a large number of concept-candidates and for various layers and models is cumbersome. To speed this up, we propose \emph{Automatic Concept Annotation} (\emph{ACA}) method that makes use of various human-defined concepts to perform a first pass on the concept-candidates. A human is then bring in the loop to add further fine-grained information about each cluster and to annotate unannotated clusters. In the following, we describe the method in detail.

\paragraph{Automatic Concept Annotation (ACA)}
ACA works in two steps: 1) 


==> methodology.v1.tex <==
Consider a neural network model $\modelM$ with $L$ layers ${l_1, l_2 , ..., l_L}$. Our goal is to analyze latent concepts learned in a layer $l_j$ of $\modelM$. Let $\dataD$ be a dataset composed of $S$ sentences where each sentence consists of $M$ words $w_1, w_2, ..., w_M$. We extract layer-wise contextualized representation of each word $w_i$ in sentences $S$.\nd{Are you going to describe the method/model formally? The notation looks strange otherwise.} In the case of a word split into subwords, we use mean pool over the subwords to create contextualized embedding of the word.\nd{This is a trivial detail which is disturbing coherence. Move it elsewhere or footnote}
%
For each layer, we cluster words into $K$ groups using \textcolor{red}{agglomerative hierarchical clustering} \sout{their} \textcolor{red}{trained on the}  contextualized \sout{representations} \textcolor{red}{feature embedding}. 
%We use agglomerative hierarchical clustering with \textcolor{red}{average linkage}. 
We refer to these groups of words as \emph{concept-candidates}. Each concept candidate \textcolor{red}{re}presents a latent concept that the model has learned about the language. We prepare an annotation schema and manually annotate 
%The next step is to 
the concept-candidates based on our definition \sout{of concept} \textcolor{red}{in} (Section~\ref{sec:concept}). In the following subsections, we provide details of each step.

\subsection{Concept Candidates}

\paragraph{Data}

\nd{This section is not part of the method. Even if it is, it is looking more like a limitation of the method rather than methodological detail. I would move these details to the experimental settings, if not at least move it to the end of this section.}

The selection of a dataset for concept analysis is of prime importance for several reasons. A small dataset from a particular domain would likely to result in domain-specific clusters.\nd{We don't know this to be completely true. There will be some language clusters that will be robust to domain shift. Again I see this more self-damaging} Similarly, high frequency tokens may dominate the low frequency tokens in clustering. 
%
The size of the dataset is another factor to be considered here. Ideally, one would like to form latent clusters over a large collection of diverse text. However, clustering a large number of high-dimensional vectors is computationally and memory intensive. For instance, 200k vectors each of size 768 require around 400GB of memory. A potential workaround is to reduce the dimensionality of words before clustering. However, this may cause a loss of information and the resulting clusters may not be a true representation of the latent space of BERT.

We \sout{handle these points} \textcolor{red}{address these problems} by starting with a large dataset of News 2018 WMT\footnote{\url{http://data.statmt.org/news-crawl/en/}} (359M tokens/types). We randomly select 250k sentences ($\approx$5 million tokens). We further limit the number of tokens to $\approx$210k by discarding singletons, closed-class words, and restricting tokens to a frequency of maximum 10 occurrences.
 
\nd{Data section should be rewritten with this last paragraph as the opener and then softening the domain issue and frequency issue in the second paragraph}

%
%The final dataset consists of 210k tokens and 77k types belonging to 250k sentences. 
%We want to consider a reasonable size vocabulary with multiple contextualized representations of a word vectors representing each word to 
%
For every token, we extracted its contextualized representations and embedding layer representation using BERT~\citep{devlin-etal-2019-bert}. 

\begin{figure}
    \centering
    \includegraphics[scale=0.3]{iclr2022/figures/elbow.png}
    \caption{Elbow}
    \label{fig:elbow}
\end{figure}


\paragraph{Clustering}
We use Agglomerative clustering\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.cluster.AgglomerativeClustering.html}} with \textit{affinity=euclidean} and \textit{linkage=ward} to cluster representations of a layer. The number of clusters $K$ is a hyperparameter. We found an optimal value of $K=1000$ using the Elbow \textcolor{red}{**cite} method. Figure~\ref{fig:elbow} shows the Elbow scores over a range of cluster values.\nd{More details needed} 
\nd{This section needs to be bloated. Do we not have a model that we can describe formally?
May be explain euclidean and linkage settings. }

\subsubsection{Annotation Task}
Following our definition of a concept, we asked two questions from the annotators:

\begin{enumerate}
    \item[\texttt{Q1}:] Is the cluster meaningful?
    \item[\texttt{Q2}:] \sout{Given} \textcolor{red}{Can the} two \textcolor{red}{sibling} clusters\sout{, do these clusters} \textcolor{red}{be combined to} form a meaningful group\textcolor{red}{ if combined}?
\end{enumerate}

\texttt{Q1} \textcolor{red}{mainly involves identifying if the cluster is human interpretable, according to our definition of a concept (Section \ref{sec:concept}), opening a category where it belongs or classifying it into an appropriate existing category}.
\sout{is mainly targeting our definition of a concept. } In \texttt{Q2}, we \sout{provided siblings as two clusters}
\textcolor{red}{asked the annotators to identify whether two sibling clusters can be combined to form a meaningful cluster as well}. Our motivation is to keep the hierarchical information \textcolor{red}{that BERT is capturing} intact. \sout{for cases where annotators agree that two siblings would result in a meaningful cluster.} \textcolor{red}{For example, a cluster capturing Rock music band in the US can be combined with its sibling that learns Rock music band in the UK to form a Rock music band.}
\sout{An answer of \texttt{yes} to each question prompted the annotator to suggest one or more possible labels for the cluster (in the case of \texttt{Q1}) or the resulting cluster when combined two siblings (in the case of \texttt{Q2}).} 
\sout{For both \texttt{Q1} and \texttt{Q2},} We provided contextual information of the words \sout{in the form of a mouse-hover feature} \textcolor{red}{for each of these questions. Having contextual information enables very fine-grained concepts, for example named entities:person can be classified into finer named-entities:person:Hollywood.} \sout{This enables discovery of syntactic clusters e.g. position of words in a sentence.} The annotation instructions combined with the examples and a screenshot of the annotation platform is provided in Appendix \ref{ssec:appendix:annotation}.

The concept-candidate annotation \sout{has been done} \textcolor{red}{is carried} by three annotators \sout{and disagreed cases were resolved in a consolidation discussion} \textcolor{red}{followed by a consolidation step to resolve disagreements}.
% We used three annotators per concept-candidate and resolved the cases of disagreement in a consolidation discussion. 
The annotators \sout{are} \textcolor{red}{were} asked to \sout{keep the} \textcolor{red}{maintain} hierarchy \sout{information intact} while annotating e.g., a cluster of ice hockey will be annotated as \texttt{semantic:entertainment:sport:ice$\_$hockey} since the words are semantically grouped and the group belongs to sports, which is a subcategory of entertainment. In case of more than one possible properties that form a cluster, we annotate it with both properties e.g., title case and country names where the former is a lexical category and the latter is a semantic category.

\subsection{Concept Labels}

We define a hierarchical concept-tagset, starting with the core language properties i.e., semantics, parts-of-speech, lexical and syntax. In order to minimize human bias in defining the tags, we assign the core properties a cluster belong to, and evolve the fine-grained tagset with the annotation process. \nd{I did not get this point. How will that minimize human bias. Also what do you mean by human bias here is not clear}?
%We additionally introduce a few lexical and syntactic tags that can be automatically annotated such as, cluster of words occurring as first word or last word in a sentence, casing, common suffix and prefix, etc. 
It is worth noting that the core language properties are not mutually exclusive i.e., a cluster can belong to more than one core properties at the same time.\nd{we just said this a few lines ago in the previous section and also before} 

Consider a group of words mentioning \textit{first name} of the \textit{football players} of the \textit{German} team and all of the names occur at the \textit{start of a sentence}, the following series of tags will be assigned to the cluster: \texttt{semantic:origin:Germany}, \texttt{semantic:entertainment:sport:football}, \texttt{semantic:namedentity:person:firstname}, \texttt{syntax:position:firstword}. Here, we preserve the hierarchy at various levels such as, sport, person name, origin, etc., which can be used to combine clusters to analyze a larger group. Appendix \ref{ssec:appendix:concept_labels} provides a complete list of tags with examples.


